Crowdsourcing for Reminiscence Chatbot Design

In this work-in-progress paper we discuss the challenges in identifying effective and scalable crowd-based strategies for designing content, conversation logic, and meaningful metrics for a reminiscence chatbot targeted at older adults. We formalize the problem and outline the main research questions that drive the research agenda in chatbot design for reminiscence and for relational agents for older adults in general.

==> sections/actions-requirements.tex <==
\begin{easylist}
\ListProperties(Hide=100, Hang=true,Style*=\textbullet~)
& \textbf{Eliciting information}. Posing questions about the life of the person, using the pictures as triggers.

& \textbf{Bringing up engagement content}. Bringing up multimedia material that will help elicit information

& \textbf{Showing understanding}. Posing comments that show understanding of the conversation content, and the user input. 
%Comments on the pictures can be generally classified to: 
% i) appreciation (e.g “Such a nice picture!”, “Um. Sounds interesting”), 
% ii) opinion (e.g “i think is a beautiful panorama”, “I think, I believe, it seems”) 
% iii) Thanking (“Thank you for sharing that with me! ”) 
% iv) Backchannel (“oh”, “right” , “ok”, “yes”)[ref. Stolcker et al. 2011] 

& \textbf{User engagement inquiry}. Posing questions to check the user engagement, and testing potential topics to address next (e.g. would you like to talk about your hometown, Moscow?)

%& \textbf{Reconnection inquiry}. Posing questions to probe potential reconnections. Unlike eliciting information, these questions are designed to test the possibility of connecting this individual with other users based on commonalities.

& \textbf{Recovery}. This action should be triggered when the bot has made an incorrect assessment in the conversation, potentially pointed out by the user. A recovery strategy should help redirect the conversation in the direct path.

& \textbf{Protocolar} General responses such as:
Conversational-Closing (“Well, it’s been nice talking to you”); Greeting (hello {"name"}!); Signal non-understanding  (“Excuse me?”)

\end{easylist}




Actions of the bot that are not visible to the user:

\textbf{Deciding on next action, state tracking}.

\textbf{Updating user profile info}. Every time when new information relevant for user profile is obtained, it should be saved in the knowledge base, therefore the bot will not ask the same things twice and user information can be used on the next turns of the conversation.

\textbf{Generating response}

The decision on choosing the next Dialog action is based on the current State of the conversation and possibly checking the Knowledge Base (see Figure1).

For our case of the conversational reminiscence bot, at each new dialog turn following parameters has to be checked:

i) Current context (macro, micro )

ii) Knowledge about: 

the user (set of attributes from the user Profile already retrieved);

the  pictures (set of tags about picture, if any pictures was uploaded previously by the user);

iii) previous user act (e.g picture uploaded/ or not)

iv) history of conversation (topics/subtopics already discussed)

\subsection{Requirements}

In this section we  identify a set of requirements that the bot should met, in order to be: i) engaging and ii) succeseful in terms of eliciting and using information about the user profile. 


(i) \textit{long term memory on the user profile}

Ability to elicit the information on the User Profile during conversation and store it, to use this knowledge about user on the next turns of the conversation.

(ii) \textit{history of conversation}

Ability of the bot to remember the history of conversation, current context and topics already discussed.

iii) \textit{Retrieving information from pictures}

Ability of getting information on what is on the pictures submitted by the user (labels) and which sentiment the picture have.

As the reminiscence therapy approach rely heavily on the use of pictures as a triggers for bringing the memories of older person, system needs to have an ability of recognizing the user's digital pictures.

iv) \textit{Flexibility}

Chatbot needs to understand the user utterances on topic in a different phrasings, both: the user responses to questions about the past from bot, and new  information the user decided to tell by himself. 

v) \textit{Sentiment tracking} 

vi) \textit{Switching context}

The ability of the bot to decide if to keep the topic of conversation or to switch to another one, while the reason can be different: sad or negative sentiments of user, the fact that topic has been fully explored, or the user has submitted new information and  the transition is more natural than staying on the current topic. 

In the next Section we frame the requirements for the system into the list of Actions the bot should be able to perform. 





\textbf{Why is it hard to met this requirements? Where and How the crowd can help?}

